Connecting the Dots: Computer Systems Education using a Functional Hardware Description Language

A functional hardware description language enables students to gain a working understanding of computer systems, and to see how the levels of abstraction fit together. By simulating circuits, digital design becomes a living topic, like programming, and not just a set of inert facts to memorise. Experiences gained from more than 20 years of teaching computer systems via functional programming are discussed.

==> eptcsdata.tex <==
\providecommand{\firstpage}{20}
\providecommand{\publicationstatus}{M. Moraz\'an and P. Achten (Eds.): Trends in Functional \\ Programming in Education 2012 (TFPIE 2012).\\
EPTCS 106, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.106.2}{10.4204/EPTCS.106.2}}
\pdfoutput=1

